Functional Dynamical Structures in Complex Systems: an Information-Theoretic Approach

Understanding the dynamical behavior of complex systems is of exceptional relevance in everyday life, from biology to economy. In order to describe the dynamical organization of complex systems, existing methods require the knowledge of the network topology. By contrast, in this thesis we develop a new method based on Information Theory which does not require any topological knowledge. We introduce the Dynamical Cluster Index to detect those groups of system elements which have strong mutual interactions, named as Relevant Subsets. Among them, we identify those which exchange most information with the rest of the system, thus being the most influential for its dynamics. In order to detect such Functional Dynamical Structures, we introduce another information theoretic measure, called D-index. The experimental results make us confident that our method can be effectively used to study both artificial and natural complex systems.

==> 2_ComplexDynamicalSystems.tex <==
\chapter{Complex Dynamical Systems} 

\epigraph{It may happen that small differences in the initial conditions produce very great ones in the final
phenomena}%
{Henri Poincar\`e}

\vspace{0.5cm}


\indent As stated in the introduction, we study the dynamical organization of complex systems using methods based on information theory. To do so we model a system using a random field from a complex dynamical systems theory perspective. This theory is an extension of dynamical systems theory, which considers system describing by few variables, to complex systems which are described by a huge numbers of variables.       
Complex dynamical systems theory provides theoretical models to describe properties like self-organization, nonlinearity, stability and change which characterize the dynamical organization of complex systems. Hence, understanding the basic concepts of this theory is needed in order to study complex systems. In this chapter, we present the definition of dynamical system, we introduce the notions of stability and attractor. Furthermore, some notions about chaotic systems and bifurcation theory are presented.  


==> 7_Appendices.tex <==
\begin{appendix}
\chapter{Mathematical Notation}


\end{appendix}
